Explaining with Examples: Lessons Learned from Crowdsourced Introductory Description of Information Visualizations

Data visualizations have been increasingly used in oral presentations to communicate data patterns to the general public. Clear verbal introductions of visualizations to explain how to interpret the visually encoded information are essential to convey the takeaways and avoid misunderstandings. We contribute a series of studies to investigate how to effectively introduce visualizations to the audience with varying degrees of visualization literacy. We begin with understanding how people are introducing visualizations. We crowdsource 110 introductions of visualizations and categorize them based on their content and structures. From these crowdsourced introductions, we identify different introduction strategies and generate a set of introductions for evaluation. We conduct experiments to systematically compare the effectiveness of different introduction strategies across four visualizations with 1,080 participants. We find that introductions explaining visual encodings with concrete examples are the most effective. Our study provides both qualitative and quantitative insights into how to construct effective verbal introductions of visualizations in presentations, inspiring further research in data storytelling.

==> section/pre-discussion.tex <==
\section{Discussion}
% interesting examples increase the attention - The Effects of Interesting Examples and Topic Familiarity on Text Comprehension, Attention, and Reading Speed
 
Comparing the results from Study 2 (Mekko chart) and Study 3 (connected scatter plot), we found an effect of introduction type on comprehension when people viewed the Mekko chart, but no such effects for the connected scatter plot. 
Our regression analysis, which additionally accounts for the effects of visual literacy on performance, revealed that people relied more on their visual literacy when interpreting the connected scatter plot above and beyond the introduction. 
However, this was not the case when people viewed the Mekko chart, which suggests that the introduction was able to help people comprehend the Mekko chart better despite their varying visual literacy levels. 
This may imply that the Mekko chart we used in our study was more complex to interpret than the connected scatter plot, pushing people to follow the introductions than relying on their existing knowledge. 
We can find further evidence by comparing the overall performance on the comprehension test for the two charts, as shown in \autoref{fig:study2aand3a}. Participants performed significantly better on the comprehension test when they viewed the connected scatter plot than the Mekko chart ($F = 13.07, p = 0.0004$), which suggests the connected scatter plot was easier to comprehend than the Mekko chart.

This may suggest that introduction plays a even more critical role when people cannot rely on their existing knowledge to decipher the visualizations. Our results echo the findings in Tanahashi et al.~\cite{tanahashi2016study}, who examined online guide designs that educate users on how to utilize information visualizations. They experimented with four visualization types --- node-link diagram, scatter plot, storyline chart, and tree map, and found guides that present a broad overview before providing details to be the most effective in all visualization types except the node-link diagram. They found no significant effects of guide designs for the node-link diagram, and believed the reason to be that participants were familiar enough with the node-link diagrams from similar, everyday visualizations like star constellations and train/subway maps. This familiarity likely overshadowed any effects of guide designs in Tanahashi et al., and we suspect the same mechanism is at work in our connected scatter plot study. 

Learning science researchers categorize instructional materials into two approaches: top-down and bottom-up. Top-down approaches start with an overview before diving into the details, while bottom-up approaches start with detailed examples and then conclude with a summary ~\cite{lovrich2007classroom}. In the context of this paper, introductions that begin with an indicator take the top-down approach, while introductions without indicators are more similar to a bottom-up approach, but without the summary. Based on the Mekko chart studies, although existing works have typically found a beneficial effect of using the top-down approach in writing \cite{kieras1978good} and introductory materials \cite{tanahashi2016study}, we found that the top-down approach is only better when the instruction does not include details and concrete examples. Namely, an introduction with the indicator component is only more effective than its counterpart (without the indicator component) when the introduction does not include a knowledge component. When detailed examples are included in an introduction as the knowledge component, not including an indicator is better when presenting a Mekko Chart. 

We turn to literature in educational psychology to resolve the seemingly contradictory findings between our Mekko chart case study and some existing literature. The length of the introduction has been shown to interact with the existence of indicators (e.g., topic sentences) to influence how people process verbal information. For example, when the text is short, including indicators (e.g., overviews and summaries) improves people's ability to recall more relevant content from a piece of text. But when the text is long with a large amount of details, including an indicator does not help people recall more relevant content from the text \cite{lorch1996effects}. This suggests that while indicators seem to enhance cognitive process of text information, there exists a length---detail trade-off such that the beneficial effect of indicators diminishes with greater amount of verbal information. Each component of the introduction are competing for human cognitive resources \cite{clark2011efficiency}. The results from our Mekko chart case study seem to suggest that it is beneficial to exclude the indicator component in an introduction, to free-up the cognitive resources for the visualization viewers to process the knowledge components.

\subsection{Limitation and Future Directions}
\label{limitation}

\subsubsection{Other Introduction Types} 
Our classification system from Study 1 mapped out a large design space of introduction types. The present paper only investigated a subset of them, but future research can continue exploring this space. For example, we only compared the effectiveness of the three explanation component subcategories on comprehension in Study 2A and 3A, and we only included the best performing explanation type in our introduction type evaluation in Study 2B and 3B. %Additionally, we only explored using extrema as the knowledge component. 
Future work could evaluate the effect of other indicator subcategories and the other introduction structures on comprehension.

\subsubsection{Other Visualizations and Dependent Measures} 
The present study investigated introductions for Mekko charts and connected scatter plots as two case studies, because we identified these two visualizations as having the desirable complexity for the purpose of our investigation. Future researchers could continue to explore the space of visualization complexity. % to further identify visualization types that demonstrates ``desirable complexity." 
In education research, ``desirable difficulties" is used to describe tasks that are just hard enough to slow down one's initial processing of the information \cite{diemand2011fortune}. This slow initial processing may hurt immediate performance and comprehension, but encourages long-term retention of the information \cite{bjork2011making}. We envision a parallel can be drawn with visualization complexities to achieve a desirable complexity. In this case, a visualization viewer would be forced to slowly process the components of a visualization to encourage long-term retention and comprehension of the visualization. With a newly defined design space of visualization complexity, future researchers could further explore how different introduction approaches affect visualization comprehensions across a wider range of visualization designs. 

Further, the present studies accessed the effectiveness of visualization introductions only via comprehension questions adpated from \cite{lee2016vlat}. The effectiveness of introductions (or other narrative techniques) can also be evaluated by measuring their effect on audience engagement \cite{boy2015storytelling}. We chose a more objective approach to measure comprehension in order to generate visualizations that improves understanding, but future researchers can also investigate the effect of these introductions with other dependent variables such as visualization content recall or audience engagement. 

\subsubsection{Beyond Crowdsourcing}
We analyzed crowdsourced introductions to gain knowledge of which introductions people consider effective, and we evaluated variations of the introductions extracted from the crowdsourced approaches. For the current study, we did not consider other, less intuitive approaches to introduce a visualization, such as using colloquial language to tell an engaging narrative, as seen in \cite{kerby2018fusion}, or using text-book like technical expository introductions, as seen in \cite{lorch1996effects}. A recent study have found that engaging narrative introductions to a piece of text makes the content more memorable for readers \cite{mensink2020effects}. We encourage future researchers to investigate these other types of introductions, and their effect on the audience beyond comprehension. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Design Implications}
Our classification system based on crowdsourced introductions can be used as a library for presenters to compose visualization introductions. We recommend presenters to try different approaches in their introductions, such as experimenting with types of \textit{explanation}s (e.g., encoding, rule, or referent) and \textit{indicator}s (e.g., abstract, topic, or theme). A presenter can also provide \textit{knowledge} with different examples (e.g., extrema, trends, etc.). We also caution visualization presenters about the length---detail trade-off. Our Mekko chart case study suggests that including the explanation and knowledge components in a introduction yields the most promising result. Including both the indicator and knowledge component seem to hurt performance, likely because the introduction becomes too length with both and cognitive-resource demanding.

We emphasize that the introductory description we examined in the present study is only one among many techniques a presenter can use to enhance the clarity of their visualization presentation. Other rhetoric techniques, such as animated transitions \cite{wang2018narvis}, repetitions \cite{mayer2008revising}, and annotations \cite{hullman2011visualization}, are all tools to smarten a Slide Show up.

%has identified different approaches to give an introduction of a visualization. 
% For example, the presenter can use three approaches, namely, \textit{encoding}, \textit{rule} and \textit{referent} to explain a visual channel.
% Presenter should not be limited to certain toolkit when guiding people through the visualization.
% Our experiment results recommend to giving concrete examples (knowledge components) when explaining the visualization.
% Meanwhile, our recommendation is compatible with implications of previous research on how to introduce a visualization.
% Examples include giving a knowledge component by first asking the audience a question about it~\cite{tanahashi2016study}, giving an explanation when only show related components of the visualization~\cite{wang2018narvis} and giving a knowledge component with related region of the visualization highlighted~\cite{wang2018narvis,kong2019understanding}.
% The last implication is about the trade-off between including both the indicator and the knowledge.
% If the introduction is too lengthy because the visualization is complex, we suggest the presenter exclude or minimized the indicator component (e.g., giving the abstract type indicator such as ``Let me introduce you a visualization") to let the audiences can assign their cognitive resources to processing the knowledge instead of information from the indicator. 
% Moreover, when the time is limited, it would be better if presenters prioritize giving examples and shorten time spending on indicator.
% \cx{Here also talk about how ppl can combine our recommendations of using E+K with the techniques you introduced in the related work section (e.g., using animations, decomposing a visualization, etc) to make their presentation even better! }
% To avoid the effects of external confounding variables such as the participants' prior belief, we removed text labels explaining the meaning of the x-axis, y-axis, and, the color legend of charts in our experiment. Participants can only rely on the audio narration to understand the chart.
% Yet, in real life scenarios, some other factors could affect the audiences' comprehension.
% For example, Mayer and Johnson~\cite{mayer2008revising} found that showing short redundant phrases of the presenters' narration when playing the slideshows enhanced the audience' memory to the content than not showing any text in the slides.
% Future works can investigate the interaction of the introduction types and other factors of a presentation such as the text information in the slides.


% limitations not included in CHI submission
%We do not give text information which is not mimicking the real scenarios \cx{Cindy: I forgot what this one is about?}
% \subsubsection{Impact of Other Factors in Oral Presentation}
% To avoid the effects of external confounding variables such as the participants' prior belief, we removed text labels explaining the meaning of the x-axis, y-axis, and, the color legend of charts in our experiment. Participants can only rely on the audio narration to understand the chart.
% Yet, in real life scenarios, some other factors could affect the audiences' comprehension.
% For example, Mayer and Johnson~\cite{mayer2008revising} found that showing short redundant phrases of the presenters' narration when playing the slideshows enhanced the audience' memory to the content than not showing any text in the slides.
% Future works can investigate the interaction of the introduction types and other factors of a presentation such as the text information in the slides.

% Moreover, crowdsourced participants and the general public are not equivalent groups.
% Although our participants varied across different age groups, education and visualization literacy levels, our study biased towards people who would join research studies online. 
% Future studies can investigate how to write effective introductions from the eyes of a more diverse public group.
% We can explore potential collaborations with local governments or news outlets.

% 1. Crowdsourced introductions are not the best ->  we evaluated what's best among what ppl currently do. But there could be better introduction styles that ppl are not aware of (and thus we didn't observe examples in our crowdsourced introduction samples).
% 2. Crowdsourced participants != the general public. Although our participants varied across different age group and education levels and visual literacy, we are biasedly selecting for people who would complete research studies online. Future studies can further investigate how to write an introduction for a even more general public can explore opportunities to collaborate with local governments or news outlet, etc. 

% \subsubsection{Individual differences} 
% We also found individual differences in our studies where participants' visualization literacy, gender, age, and education level all have differing effects on comprehension.
% This can be related to our findings about study1 that crowdsourced participants took different approaches to give introductions.
% It indicates potential benefits of individually tailored introductions that accounts for people's background, prior knowledge and demographics. Although this would not fit into the live presentation with diverse audiences, it can benefits individual or small-group presentations which involves more interactions between the presenter and the audience and requires presentation tools to be more flexible ~\cite{kosara2013storytelling}. 
% we examined visual literacy, and found positive effects on comprehension
% there also seems to be effects of age and education
% also in study 1  crowdsource ppl took different approaches,
% there may be a benefit of individually tailored introductions that accounts for people's prior knowledge. Although this won't work well in a general presentation, in personal communications, such as researcherrs explaining a visualization they made with peers, might be helfpul.
% Can tie back to this reference in the related work - Kosara and Mackinlay~\cite{kosara2013storytelling} further defined three storytelling scenarios: self-running presentation, live presentation in front of an audience, and individual or small-group presentations. 

% \subsubsection{Introduction Text Classification System}
% \leni{it seems like an over claim}
% We take the first step towards segmenting and classifying visualization introductions and propose a classification system.
% In future we hope to utilizing natural language processing techniques automatically generate introductions for visualizations.  
% It requires collecting large amount of introduction data and a more fine-grained classification system presenting more linguistic features of % visualization introductions.

% Limitations:
% 1. The skewed age distribution of the participants
% 2. We can not make sure every participant gave much efforts
% 3. We did not discuss what kinds of knowledge are most effective: (a) it depends on the chart (b) could be another study out of the scope of this paper.
% 4. We don't cover different data 
% 5. In real scenario, the charts would be accompanied with text. We can mention the work "Understanding Visual Cues in Visualizations Accompanied by Audio Narrations" which found people rely to the audio according to their interview and argue that the experiment results still have practical implications.
% 6. Did not evaluate combinations of different types of explanations
% 7. may have failed due to the simple fact that people have a limited attention span on the internet, and that if they read through an introductory narrative component, they will not spend extra time exploring a visualization -> paper shows the importance of time.


% Old version
% The study results indicate that for Mekko chart, introduction types containing the knowledge component can substantially improve participant performance than other types.
% However, for connected scatter plot, there is no significant difference between introduction types.
% When reading connected scatter plot, the visualization literacy becomes the significant factor that decides participant performance.
% While reading Mekko chart, the effect of visualization literacy was no longer significant.
% In this case, participants can not rely on their visualization literacy to do the comprehension test and the introduction plays an important role in their comprehension.
% We assume that is because the connected scatter plot is easier to be understood than the Mekko chart.
% Therefore, as long as the introduction explains what data is encoded in the chart, people understand it by their prior knowledge.
% Similar result was found in the work of Tanahashi et al.~\cite{tanahashi2016study}.
% They compared four ways of adding exercise questions into the introduction materials of visualization, and found significant difference between these ways in affecting participants' comprehension of most visualizations except for node-link diagrams.
% They believed the participants were already familiar with the node-link diagrams as people see similar visualizations like star constellations and train/subway maps in everyday lives across various cultures.

% In terms of the indicator component, although we observed people typically included it in the introduction, it did not significantly improve the effectiveness of the introduction.
% Research from educational psychology found that giving headings has less influence on recall the topics of text at greater length with more details than on recall the topics of text at shorter length~\cite{lorch1996effects}.
% As the function of headings and indicator are both about summarizing the information, the reason why we did not find significant effect of indicator could be that the knowledge or explanation components gave enough details about the visualization and attract more attention.

% We also observed a trade-off between indicator and knowledge.
% When the introduction of Mekko chart including both indicator and knowledge components hurts the performance while including only one of them improves the performance.
% However, such trade-off was not seen in introductions of the connected scatter plot.
% Based on theory from the science of learning, understanding the visualization from indicator component is a top-down learning in which knowledge is given abstractly and understanding the visualization from knowledge component is a bottom-up learning in which knowledge is extracted from details~\cite{lovrich2007classroom}.
% When both indicator and knowledge components are included, there is an interaction between top-down and bottom-up learning and previous research has found that people's actual learning direction may be either one or mix of the two depending on many variables~\cite{sun2004top}.
% Meanwhile, there is no conclusion of which approach is the most effective~\cite{Sun2012}.
% In our case, when the visualization is complex, emphasizing the bottom-up approach, that is putting more efforts on designing the knowledge component instead of the indicator component is preferred.

==> section/pre-introdcution.tex <==
Imagine a data analyst sharing the latest findings in a presentation to some stakeholders. %speaker is going to tell insights about a data in an oral presentation. 
When preparing the presentation, the analyst decided to use a data visualization to illustrate an interesting data pattern to engage the stakeholders. 
The analyst considered simple charts such as bar charts, line charts, and pie charts, but they can only encode a limited number of data dimensions.
The analyst, an expert data visualization specialist, designed a visualization that illustrates several data dimensions using multiple visual encoding channels, following the state-of-the-art design practices. 
During the presentation, the analyst excitedly shows the visualization to their audience, emphasizing how the data patterns connect to a recent strategic move in the company.
However, the visualization was delivered too quickly without a proper description to guide the stakeholders through its components, leaving everyone overwhelmed and confused.

This phenomenon, known as the \textit{curse of expertise}, where background knowledge makes it difficult for experts to take the perspective of a novice, has been replicated in research labs \cite{xiong2019curse}. 
Visualization presenters can often confuse their audiences when they deliver complex information too quickly or when they provide too few details.
They might not realize that their audiences may not have the same degree of familiarity with the visualization. 

With the ability to communicate data stories intuitively and engagingly, 
data visualizations are becoming increasingly prevalent in verbal presentations.
Using novel visualization techniques, such as connected scatter plot and streamgraphs, can make the presentation more memorable and engaging. But it may also be more confusing for the audience~\cite{kosara2016presentation}.
Without proper guidance, people might give up reading an unfamiliar visualization if it requires extensive mental effort and motivation~\cite{lee2015people}.
Therefore, it is critical to walk the audience through the visualizations in a presentation so they can easily see and understand the patterns in data. 

An effective introduction should guide the audiences through the visualization set-up, allowing them to follow the presenter's story and easily see the data patterns the presenter references. 
This may require the presenter first to walk through the visualization components \cite{wang2018narvis}, identify the visual encoding channels and explain what each visual mark represents.  Therefore the audiences can follow the logic of the presenter when the presenter provides data insights based on the visual patterns.
The introduction may also benefit from the topic and concluding sentences, as well as examples \cite{kieras1978good}, but it should be concise enough to keep the audience attentive.
However, the presenter may struggle with what kind of information to include in the introduction to maximize clarity,
as the presenter has more background knowledge of the visualization than their audience, general audiences, and their curse of knowledge makes it hard for them to think from the audiences' perspectives.

This motivates us to investigate the critical information a presenter should include in a visualization introduction during a presentation to be informative and concise. 
These studies suggest that we need more knowledge on what information is expected by the general audiences in an introduction of a visualization.

% In Study 1, we \cx{investigate how visualizations would be introduced in verbal presentations.}
% \cx{We collected visualization introductions from crowdsourced participants and analyzed their response. We generated several types of introductions based on these introductions and evaluated their effectiveness in Study 2.}

% We dissected the 112 introductions we collected, segmenting and classifying them into three major components - \textit{Indicator}, which states the goal or summarizes the introduction, \textit{Explanation}, which illustrates how visual encoding channels map on to the data values, and \textit{Knowledge}, which describes facts and insights from the visualization. Each of the three major components were also subcategorized and clustered by their key features into finer variations. we report one features of introductions from the participants

% In Study2, we constructed different versions of introductions and compared their effectiveness in facilitating the understanding of visualizations in two experiments.
% Participants first viewed a visualization while listening to one version of the introduction and then answered comprehension questions about the visualization.
% We examined which version most effectively introduces a visualization by comparing their performance on the comprehension questions.
% In this first experiment (Study 2a), we compared the effectiveness of introductions using different kinds of \textit{Explanation}. 
% In Experiment 2, we evaluated introductions varied in structures. 
% Their difference lies whether the \textit{Indicator} or \textit{Knowledge} component is included in the structure, and how the \textit{Knowledge} and \textit{Explanation} components are integrated.
% We found  to be the most effective. 

==> section/pre-study2.tex <==
\section{Study 2A: Explanations for A Mekko Chart}
In Study 1, we segmented introductions into three major components: \textit{indicator}, which states the goal or summarizes the introduction, \textit{explanation}, which illustrates how visual encoding channels map on to data values, and \textit{knowledge}, which describes facts and insights from the visualization. Each of the three major components was also subcategorized and clustered by their key features into finer variations. Therefore, each component can be written with a different approach. For example, as discussed in \autoref{code_system}, an explanation component can be written in at least three ways: referent, encoding, and rule. In this study, we compare the three approaches to \textbf{the explanation component} to examine which is the most effective at facilitating people's understanding of visualization.

In Study 1, participants performed the worst in writing three findings they observed from the Mekko chart compared to other visualization types (average number of correct answers: Mekko chart:2.08, connected scatter plot: 2.36, sorted stream graph: 2.55, and waterfall chart: 2.46). % the average number of correct findings people wrote about the Mekko chart is the least compared to those about the other three charts
Therefore, we chose to show participants a Mekko chart with an explanation in this study to avoid ceiling effects, so that fewer participants could understand the chart and correctly answer all the comprehension test questions without any introduction or explanation. 

\subsection{Study Design and Procedure}
In this between-subject study, participants were randomly assigned to listen to one of three explanation types (referent, encoding, rule) while viewing a Mekko chart. They were told to think of the audio as a presenter introducing the Mekko chart during a presentation. After the explanation audio ends, the participants completed a comprehension test with eight questions about the Mekko chart they saw. % 3 groups in which, each group of 30 participants were assigned to a particular \textit{Explanation} type explaining one chart. In the experiments, participants first viewed a visualization accompanied by one version of the introduction and then took a comprehension test with eight questions about the visualization. As this study targets oral presentation scenarios, the introduction was given through an audio narration. We compared participant performance on the comprehension test as the metric to compare the effectiveness of different introductions. We selected the Mekko chart as the visualization.
% \subsubsection{Study procedure}
% We conducted the between-subjects experiment and every participant is randomly assigned one introduction type. Participants first read the experiment instruction and were told to imagine they were listening to a presentation where visualization is introduced. Then participants were requested to understand the chart by following the accompanying audio and took the comprehension test after the audio is finished.
The comprehension test questions were presented one at a time in random order. %had one question per page and the order of questions was randomized.
Participants were not allowed to return to the previous question to change their answers. % when the page was switched.
In the end, participants completed a subjective visualization literacy assessment developed by Garcia-Retamero~\cite{garcia2016measuring}, with five items using 6-point scales, and answered some demographic questions about age, gender, and education level.
% whether they incorporated visualizations in their works, and their level of familiarity about the chart as well as the topic presented in the chart.
% The study took approximately 10 minutes and participants were compensated at a rate of \pounds 6.30 per hour. 

\subsubsection{Participants}
We recruited 90 participants (ages ranging between 18 and 70 years old, $\mu = 34.97 , \sigma = 12.88$, $51\%$ females) from Prolific~\cite{prolificwebsite}. Their mean self-evaluated visualization literacy score is 18.39 out of 30 ($\sigma = 5.28$). We filtered participants who jumped to the comprehension test section before the audio ended, finished the comprehension test too fast (completion time $Z-score < 3$), or gave wrong answers clearly indicating they did not read the questions (e.g., giving ``Jacob" as the answer for each question about the Mekko chart). We ended up with 88 valid responses. 
%\leni{The distribution of participants in each introduction type can be seen in xxx(figure-G). no need that?}

% They were directed from Prolific to Qualtrics \cx{Cite} through an external survey link to finish the experiment.
% 54 of them never or rarely incorporate data charts/visualizations in their works, 26 sometimes and 8 often or very often.
% 69 of them rarely or never saw the types of charts in the experiment, 16 sometimes, and 3 often or very often.
% \leni{don't think we have enough space in the paper}
% Detail demographic information is shown in xxx(figure-G), and details can be found in the supplementary materials.

\subsubsection{Mekko Chart Visualization}
We modified the Mekko chart from the Study 1 by removing the text labels explaining the meaning of the x-axis, y-axis, and the color legend, to ensure that participants had to rely on the audio narration to understand the chart and answer the comprehension questions. This modification was intended to prevent participants from ignoring the audio explanations and relying on their visual literacy. 
% This is to avoid that participants read the chart by themselves and infer the meaning from the text information such that the introduction does not affect their performance on the comprehension test. To estimate the effects of each \textit{Explanation} type independently from the effects of the \textit{Indicator} or \textit{Knowledge} component, the introduction only has the \textit{Explanation} component. In each version of the introduction, we wrote one sentence for explaining each visual channel of the Mekko chart. Visual channels to be explained include the height of each row, the width of each block, the color and the candidate's name. To maintain the fairness, we guaranteed each introduction had similar number of words (\textit{Referent}: 74, \textit{Encoding}: 73 ,\textit{Rule}: 86) and the time duration of the three audios are 37 seconds(\textit{Referent}), 38 seconds(\textit{Encoding}) and 44 seconds(\textit{Rule}). Details are seen in Figure xxx.

\subsubsection{Audio Explanations}
% add the data of the audio length and words count of each introduction
The audio explanations the participants listened to were designed to mimic the real-world scenario of listening to a verbal presentation. Participants were only allowed to listen to the audio once. The audio scripts for the three explanations types were composed to have parallel text complexity and length. Note that no indicator nor knowledge components were included so we could isolate the effect of the different types of explanation component only. The scripts are included below:

\textbf{Referent}: In this chart, the names of the presidential candidates are listed on the right.
On the left side, the y-axis shows each candidate’s proportional spending, with respect to the total advertising spending by all the candidates. On the bottom, the x-axis shows the percentage spent by each candidate to reach different groups of voters. The color legend on the right shows how the target voters are divided into different groups by gender and age. (Word count: 74)

\textbf{Encoding}: In this chart, each row tells us each presidential candidate’s advertising spending. For each row, the height represents the proportion spent by that candidate, with respect to the total advertising spending by all the candidates. Colors indicate different target voter groups of different ages and gender. The width of a colored block represents the proportion spent by one candidate on a specific voter group, with respect to that candidate’s spending on all groups. (Word count: 73)

\textbf{Rule}: In this chart, the rows of the presidential candidates are ordered by the width of the dark blue colored bars. The taller the row, the more the candidate spent compared to other candidates. In each row, the blue colors represent younger voters age 13 to 44, the orange colors represent voters age 45 and older. The darker color represents Men voters, and the lighter color represents Women voters. The wider the colored block, the more the candidate spent on the corresponding group of voters. (Word count: 86)

\subsubsection{Comprehension test}
We use the comprehension test scores of participants as the metric of the effectiveness of the visualization introductions.
The comprehension test consists of 8 questions, to cover a wide range of task types within a reasonable time.
The questions are based on the VLAT - the visualization literacy assessment framework developed by Lee et al.\cite{lee2016vlat}. %, which recommends testing people's comprehension of the visualization by asking them to answer questions related to different visualization tasks. 
We referenced the VLAT tasks typically used for the 100\% stacked bar chart to derive the comprehension questions for the Mekko chart. This included tasks such as \textit{Retrieve Value}, \textit{Find Extrema}, and \textit{Make Comparisons}.
In developing the questions, we noticed that the \textit{Make Comparison} questions in VLAT were True or False questions, yielding a 50\% random guessing accuracy. Thus, we modified the \textit{Find Extrema} questions to a short answer format, which requires making comparisons of multiple data value pairs instead.

We also balanced the difficulty levels of our comprehension questions following guidelines from \cite{lee2016vlat}, which ended up with 2 easy, 3 medium, and 3 difficult questions. The easy questions ask participants to retrieve specific values from the Mekko chart, such as ``What is the percentage of Claire’s advertising spending". The medium questions ask participants to make comparisons before retrieving specific values, 
such as ``Which group of voters does Jacob spend the most on?" and ``In terms of overall advertising spending, who spent the most on men voters 13 to 44?"
The difficult questions required participants to further filter for specific criteria before comparing and retrieving values, such as ``In terms of overall advertising spending, who spent most on men voters?". The questions are listed in the supplementary materials. 


\subsection{Results}
\begin{figure*}[t]
  \includegraphics[width=\linewidth]{Figures/5-study-23a.pdf}
  \caption{Accuracy for each question in three explanation types: \textit{Referent}, \textit{Encoding}, and \textit{Rule}. The upper part shows comprehension test scores for the Mekko chart (Study 2A). The lower part shows comprehension test scores for the connected scatter plot (Study 3a). The luminance represents the estimated difficulty level of the question when designing it: light gray for \textit{easy questions}, medium gray for \textit{medium questions}, and dark gray for \textit{difficult questions}. The figures indicate that participants generally performed better on the comprehension test for the connected scatter plot than for the Mekko chart.}
  \label{fig:study2aand3a}
\end{figure*}

\subsubsection{Effects of Explanation Type}
We used a one-way ANOVA to investigate any statistically significant difference between the three Explanation types. We compared the participant's performance on the comprehension test after listening to the three Explanations and found no significant effects of explanation type on the comprehension test scores ($F = 0.18, p = 0.83$). The average comprehension test scores in each explanation type were: referent (Mean = 4.68, SD = 1.96 ), encoding (Mean = 4.93, SD = 1.51), and rule (mean = 4.85, SD = 1.56). Participants seeing the encoding type performed slightly better but not significantly.
More details are shown in \autoref{fig:study2aand3a}. 

\subsubsection{Effects of Visualization Literacy}
% We need to discuss whether to show the logistic or show the linear regression results? 
We also conducted a linear regression analysis to examine the effects of visualization literacy scores from the subjective literacy test~\cite{garcia2016measuring}, age, education level, gender, in addition to Explanation type, on participant performance on the comprehension test.
The result shows that visualization literacy score is the only statistically significant predictor of performance ($coef = 0.083, p = 0.019$), where higher visualization literacy is associated with better performance on the comprehension test.
The effects of explanation type, age, gender, and education level were negligible. Details can be found in the supplementary materials.
We also compared the visualization literacy scores between participants who viewed different explanation types via a one-way ANOVA. We found no significant difference in the literacy scores between participants who viewed different explanation types ($F = 0.01 , p = 0.99$).

\subsection{Discussion}
Our results suggest that the three approaches to writing the explanation do not seem to affect comprehension differently. In other words, it does not seem to matter whether the presenter chooses a referent, encoding, or rule approach to explain the visual encoding channels in a visualization. We also see that when the instruction materials are similar enough, the participant's visual literacy levels becomes the critical determinant of how well they understand a visualization. 

Based on the coding system from Study 1, we could also investigate and compare the effectiveness of the different types of indicator components and different examples of knowledge components. However, based on the results from study 2A, we suspect the difference between each component type would, similar to the explanation component types, be negligible. We further discuss this point in our limitation section. Next, we turn our attention to the overall structure of the introduction and investigate how the three major components interact with each other to influence the overall effectiveness of an introduction. 


% Based on the coding system, we could enumerate all possible combinations of subcategories of each component, and for each combination, we could permute the components or a subset of them to generate tons of introductions. However, it is impractical to evaluate all of them. In experiment one (study2a), we only evaluated the subcategories of the \textit{Explanation} component, namely, \textit{Referent}, \textit{Encoding} and \textit{Rule}, because the \textit{Explanation} component directly reveals the visual encoding when introducing a visualization. Although some participants might think the visualization could be self-explanatory and left this component out in their introductions, it did not degrade its importance. In experiment two (study2b), we investigated how to construct an effective introduction in terms of the structure. We describe experiment one in this section and experiment two in the next section.

% Based on this, we suspect changing the approach to one component would likely have a trivial effect on the introudction as a whole. So instead, we investigate inclusion/exclusion of components in introductions. 

==> section/pre-study3.tex <==
\section{Study 2B: Introducing A Mekko Chart}

In this experiment, we investigate how the structure of an introduction affects the understanding of the visualization. We define the structure of an introduction by the existence and order of a component - whether indicator, explanation, or knowledge is included or not, and the relative order of each component.

However, permuting major components and subset of them to find and compare all possible structures is infeasible. With three components each turned on/off, the number of conditions can quickly explode. We listed the entire potential design space in our supplementary material, based on the introduction structure identified in \autoref{study1structure}. Instead, we limit our investigation scope by applying several restrictions and discuss not examined conditions in our limitations and future directions section.

First, because indicator was the most popular component, we examine whether indicators improve the effectiveness of an introduction or not. To do so, we generated instructions that include the indicator component and instructions that did not. However, we limit our investigation to when the indicator is added to the very beginning of the introduction, as it was the most popular approach, and we discuss the related limitations in \autoref{limitation}. We will also examine the effect of including versus excluding the knowledge component. But we limit our investigation to the conditions where the knowledge component follows an explanation, or is interwoven with an explanation. We made these choices because they were some of the most common introduction structure we found in Study 1. Again, we discuss the limitations of our decisions in the later sections of this paper.

\subsection{Study Design}
\label{exp2bDesign}
With these restrictions, we created six introduction structure types: explanation only (E), explanation followed by knowledge (EK), explanation interwoven with knowledge (EKEK), indicator plus explanation (IE), indicator plus explanation followed by knowledge (IEK), and indicator plus explanation interwoven with knowledge (IEKEK). Notice the last three introduction types are identical to the first three, but with an indicator added to the beginning. This set up allows us to investigate the effect of including/excluding the indicator component by comparing the first three types to the last three types. We also investigate the effect of the knowledge component by comparing (1) the introduction types that exclude the Knowledge components (E and IE), (2) the types that include knowledge but not interwoven with explanation (EK and IEK), and (3) the types that interweave knowledge and explanation (EKEK and IEKEK). % Overall, this experiment has two factors. The first factor is the existence of the \textit{Indicator} component, having two levels: including or excluding the \textit{Indicator}. The second factor is about the \textit{Knowledge} component, having three levels:(1) excluding \textit{Knowledge} component, (2) combining \textit{Explanation} and \textit{Knowledge} component as \textit{E+K+}, (3) combining \textit{Explanation} and \textit{Knowledge} component as \textit{(EK)+}.
% For convenience, we further name the first factor as "indicator existence" and name the second factor as "introduction body content" because the \textit{Explanation} and \textit{Knowledge} components are major content of an introduction.

For the introductions where the knowledge component is included but not interwoven with the explanation (e.g., EK and IEK), the explanation component explains the meaning of all visual channels. Then the knowledge component gives examples afterward. For the introduction types where explanation and knowledge components are interwoven (e.g., EKEK and IEKEK), each explanation is immediately followed by a corresponding knowledge example. Note that the resulting introduction for interwoven knowledge and not interwoven knowledge would be of the same length. 

For the explanation component, we chose the encoding type as it yielded the best results (although not significantly) in Study 2A. 
For the indicator component, we chose the topic type, which was the most commonly used type from Study 1. 
For the knowledge component, we selected the extreme data values on the chart as examples. %\textit{Find Extremum} type as examples for channels representing ordinal data and \textit{Reterive Values} type for channels representing categorical data.
For instance, a knowledge component describing the height of bars reads, ``For example, the fifth row representing Sofia is the tallest row among all rows. It means Sofia has spent more on advertising compared to other candidates." 
% about the color in the Mekko chart used "For example, the light orange represents women voters 45 and older.", and that about the height of each row in the chart is "For example, the fifth row representing Sofia is the tallest row among all rows. It means Sofia has spent more on advertising compared to other candidates.".
% In introductions with the \textit{E+K+} pattern, we first wrote Explanation components explaining all visual channel with one sentence for each and then gave Knowledge components.
% In introductions with the \textit{(EK)+} pattern we gave a \textit{Knowledge} component after each \textit{Explanation} component that introduces only one visual encoding channel in one sentence. 
% The \textit{Knowledge} components in those introductions are the same to reduce potential confounding factors.
Additionally, we ensured that the data values related to the knowledge component are not the answers to any questions in the comprehension test to maintain fairness across all six introduction types.

We provide the introduction text used in this study below, color-coded to increase the clarity in the manuscript only. The sentence within the parenthesis is the indicator. The indicators are included for three of the introduction types. They are excluded from the other three, while everything else remains the same. For example, for the first introduction below, including the indicator text in the parenthesis would yield the introduction type IE, while excluding it would yield the introduction type E. 

\textbf{(I)E}: \textcolor{indicator}{(The chart shows the proportion of advertising spent by each candidate and the percentage of advertising spent to reach specific voter groups.)} \textcolor{explanation}{Each row tells us each presidential candidate's advertising spending.
For each row, the height represents the proportion spent by that candidate, with respect to the total advertising spending by all the candidates. Colors indicate different target voter groups of different ages and gender.
The width of a colored block represents the proportion spent by one candidate on a specific voter group, with respect to that candidate's spending on all groups.}

\textbf{(I)EK}: \textcolor{indicator}{(The chart shows the proportion of advertising spent by each candidate and the percentage of advertising spent to reach specific voter groups.)} \textcolor{explanation}{Each row tells us each presidential candidate's advertising spending. For each row, the height represents the proportion spent by that candidate, with respect to the total advertising spending by all the candidates. Colors indicate different target voter groups of different ages and gender. The width of a colored block represents the proportion spent by one candidate on a specific voter group, with respect to that candidate's spending on all groups.}\textcolor{knowledge}{For example, you can see candidate names such as  Jacob, Bella, and Oliver on the right. The fifth row representing Sofia is the tallest row among all rows. It means Sofia has spent more on advertising compared to other candidates. In her row, we can also see that the light orange colored block is the widest one. As the light orange represents women voters 45 and older, it means Sofia spent more on women voters 45 and older than on any other voter groups.}

\textbf{(I)EKEK}: \textcolor{indicator}{(The chart shows the proportion of advertising spent by each candidate and the percentages of advertising spent to reach specific voter groups.)} \textcolor{explanation}{Each row tells us each presidential candidate's advertising spending.} \textcolor{knowledge}{For example, you can see candidate names such as  Jacob, Bella, and Oliver on the right.} \textcolor{explanation}{For each row, the height represents the proportion spent by that candidate, with respect to the total advertising spending by all the candidates.} \textcolor{knowledge}{For example, the fifth row representing Sofia is the tallest row among all rows. It means Sofia has spent more on advertising compared to other candidates.}
\textcolor{explanation}{Colors indicate different target voter groups of different ages and gender.} \textcolor{knowledge}{For example, the light orange represents women voters 45 and older.} \textcolor{explanation}{The width of a colored block represents the proportion spent by one candidate on a specific voter group, with respect to that candidate's spending on all groups.} \textcolor{knowledge}{For example, in Sofia's row, the light orange colored block is the widest one. It means Sofia spent more on women voters 45 and older than on any other voter groups.}

% For the \textit{Indicator} component, we evaluated whether adding it to the introduction helps.
% The \textit{Indicator} component can be found in the beginning, middle or end of an introduction.
% In this experiment, we only consider the dominant situation where the \textit{Indicator} is placed at the beginning.
% For the \textit{Knowledge} component, we evaluated whether adding it helps, as well as two most popular ways of combining it with the \textit{Explanation} component found in study1.
% The two most popular ways are (1) explaining the meaning of all visual channels with \textit{Explanation} components and then giving some examples with \textit{Knowledge} components and (2) each time only explaining a subset of visual channels and giving related examples, and repeating this procedure until all visual channels are explained, which forms multiple groups of \textit{Explanation} and \textit{Knowledge} components in the introduction sequence.
% We denote the first way as \textit{E+K+} and the second way as \textit{(EK)+}, using the same approach as study1.

\subsubsection{Participants}
We recruited 180 participants from Prolific \cite{prolificwebsite}, with age range between 18 and 72 years old ($\mu = 30.55 , \sigma = 12.42$, $61\%$ females). After applying the same exclusion criteria as that in Study 2A, we ended up with 173 valid responses. Their average visualization literacy score is 18.36 out of 30 ($\sigma = 4.90$).
% \leni{change these numbers into percentages}112 of them never or rarely incorporate data charts/visualizations in their works, 39 sometimes and 22 often or very often.
% 131 of them rarely or never saw the types of charts in the experiment, 33 sometimes, and 9 often or very often.

\subsubsection{Study Procedure}
This between-subject study follows the same procedure as study 2A. Every participant was randomly assigned to listen to one of the six types of introduction while reading the same Mekko chart from Study 2A, and answered comprehension questions. % The only difference is the audio introduction script. Instead of only including the explanation component, we used the six instruction types mentioned in \ref{exp2bDesign}.
The study took approximately 10 minutes, and participants were compensated at a rate of \pounds 6.30 per hour.  

\begin{figure}[t]
  \includegraphics[width=\linewidth]{Figures/6-study-23b.pdf}
  \caption{The average comprehension test score in each introduction type. Figure 5A shows the results for the Mekko chart. Figure 5B shows the results for the connected scatter plot. The red line represents introductions including indicator component and the blue line represents introductions excluding indicator component. The y-axis represents the average score. The x-axis represents introductions: excluding knowledge component(E), adding knowledge component following the explanation component (EK), and adding knowledge component interwoven with the explanation component.}
  \label{fig:study3ab}
\end{figure}


\subsection{Results}
%Average test scores for each visualization and IVG. The error bar shows standard error. The scores for the graph visualization are fairly even for all visualization types, which we attribute to the participants likely being more familiar with graphs. The A–T-D IVG shows a clear improvement in average score for the other visualization types.
We examined the effects of introduction types by analyzing participant performance on the comprehension test with a between-subject two-way ANOVA. The ANOVA has two factors: indicator inclusion and introduction body content. Indicator inclusion has two levels: include indicator (referring to introduction type IE, IEK, and IEKEK) and not include indicator (referring to introduction type E, EK, and EKEK). Introduction body content has three levels: no knowledge (E and IE), separated knowledge (EK and IEK), interwoven knowledge (EKEK and IEKEK). We also included the interaction term between indicator inclusion and introduction body content.

The results suggest that there is a main effect of introduction body content ($F = 4.34, p = 0.039, {\eta^2}_{partial} = 0.025$).
The average comprehension test scores in each level were: no knowledge (Mean = 5.10, SD = 1.52 ), separated knowledge (Mean = 5.72, SD = 1.53 ), and interwoven knowledge (Mean = 5.44, SD = 1.74).
Post-hoc comparison using Tukey's HSD test suggests that participants who listened to introductions with the separated explanation and knowledge components (EK, IEK) performed significantly better than who listened to introductions without the knowledge component ($p_{adj} = 0.095$). 
Surprisingly, there is no significant difference between interwoven knowledge and no knowledge ($p_{adj} = 0.50$).
There is also no significant difference between the separated knowledge (EK, IEK) and interwoven knowledge (EKEK, IEKEK) introduction types ($p_{adj} = 0.59$).

Interestingly, there is no main effect of indicator inclusion ($F = 0.45, p = 0.50, {\eta^2}_{partial} = 0.003 $), such that people did not score higher on the comprehension test when the introduction included an indicator (Mean = 5.28, SD = 1.59 ) than when the introduction did not include an indicator (Mean = 5.56 , SD = 1.63).

There is a significant interaction between the indicator inclusion and introduction body content ($F = 3.29, p = 0.07 , {\eta^2}_{partial} = 0.02 $). 
% Post-hoc comparison using Tukey's HSD test revealed a significant difference between between groups in E and EK ($F = , p_{adj} = $) as well as E and EKEK ($F = , p_{adj} = $), but no significant difference between EK and EKEK ($F = , p_{adj} = $). 
Post-hoc comparison using Tukey's HSD adjustment revealed a significant difference between introduction type E and introduction type EK, such that participants performed better on the comprehension test when they listened to introduction type E than when they did EK ($p_{adj} = 0.041$). There is also a significant difference between introduction type E and EKEK, such that EKEK facilitated better performance on the comprehension test ($p_{adj} = 0.099$). There was no significant difference in the remaining pair-wise comparisons of introduction types. Details can be found in the supplementary materials.

% The results suggest that the introduction body content factor has main effect ($F =, P =, partial \eta^2 = $). There is also a significant interaction between the indicator existence and introduction body content ($F = , P = , partial \eta^2 = $). Post-hoc comparison using Tukey's HSD test suggest that No significant effect of the factor indicator existence is found ($F = , P = $). We did two post-hoc pairwise comparison using the Tukey's HSD test to exam the effects of the introduction body content factor and the interaction. We first compared the comprehension test scores of participants who listened to introductions in \textit{IE} or \textit{E} sequences, in \textit{IE+K+} or \textit{E+K+} sequences and in \textit{I(EK)+} or \textit{(EK)+} sequences to check the main effect of the introduction body content. The results show that participants who listened to introductions with the \textit{IE+K+} or \textit{E+K+} sequence ($F =, P =, {\eta^2}_{partial} = $) performed significantly better than who listened to introductions with the \textit{IE} or \textit{E} sequence. There is no significant difference between other pairs of participant groups. Second, we conducted the pairwise comparison between participants who listened to introductions in \textit{E}, in \textit{E+K+} and in \textit{(EK)+} sequences to remove the effects of the . This time we found both significant difference between groups in \textit{E} and \textit{E+K+} conditions ($F = , P_{adjust} = $) as well as \textit{E} and \textit{(EK)+} conditions ($F = , P_{adjust} = $), but no significant difference between \textit{E+K+} and \textit{(EK)+} conditions($F = , P_{adjust} = $).

Overall, including both the explanation and the knowledge components in an introduction most strongly improves its effectiveness. %, and separating knowledge and explanation components appears to be more effective than interweaving them. 
When the introduction includes the knowledge component (interwoven with explanation or separate), adding the indicator components hurts performance. Interestingly, however, when the introduction does \textit{not} include a knowledge component, adding the indicator component improves the effectiveness of the introduction, but not above and beyond the effect of including the knowledge component.
% However, when the introduction includes an indicator component, adding knowledge hurts the overall effectiveness of the introduction. 
This suggests the knowledge component is more critical than the indicator component to be included. It may be the case that adding the indicator component competes with the knowledge component for viewer cognitive resources. Thus, including only one or the other yields enhanced results than including both. We further discuss this in the general discussion section.

% Moreover, according to the data (Figure xxx), the average comprehension scores of participants listened to introduction type IE are higher than who listened to E or IEKEK types. We conclude that the indicator and knowledge components counteract the benefits of each other, and such interaction is statistically significant when the knowledge and explanation components are interwoven.
%If the reason is because of the introduction being too long, maybe we should suggest the presenters to cut some examples instead of getting ride of the indicators; 
%As in the experiments about the connected scatter plot, the indicator components clearly have positive effects!

\subsubsection{Effects of literacy score}
We conducted linear regression analysis predicting performance on the comprehension test with the literacy score, age, education level, gender, indicator inclusion, introduction body content, and their interactions. We observed no significant effects of visual literacy on comprehension test performance ($coef = 0.03, p = 0.253$), similar effects of indicator existence, introduction body content, and their interaction as previously reported in the two-way ANOVA.
We also found effects of age ($coef = -0.0245, p = 0.018$) and gender (male = 1, $coef = -0.7088, p = 0.004$) in participant performance.
This suggests that our manipulation of the introduction types was likely effective.
The task was difficult enough for participants to rely on the introductions beyond their visual literacy. See a more thorough discussion in the general discussion section.

% Contrary to the finding in study1, in study2 there is no significant relationship between participants' performance and their visualization literacy scores ($coef = , p = $). The effects of age, education level and gender were also negligible.

==> section/pre-study4.tex <==
\section{Study 3A: Explanations for A Connected Scatter Plot}
We replicated Study 2A to further investigate the effect of the three explanation component subcategories in a new context, with a different visualization --- a connected scatter plot. This study will help us examine the generalizability of Study 2A. 

% from study1 to check the generalizability of our experiment results.

\subsection{Participants and Study Design}
We recruited 90 participants (ages ranged between 18 and 65 years old, $\mu = 31.98 , \sigma = 12.80$, $50\%$ females) and collected 88 valid responses after applying the same exclusion criteria as Study 2A. % $59\%$ of them never or rarely incorporate data charts/visualizations in their works, $26\%$sometimes and $15\%$ often or very often. $75\%$ of them rarely or never saw the types of charts in the experiment, $19\%$ sometimes, and $6\%$ often or very often.

Study 3A follows the same procedure as Study 2A. Participants listened to one of three explanations and answered comprehension questions for a connected scatter plot. The comprehension questions referenced VLAT \cite{lee2016vlat} and common misinterpretations identified in~\cite{haroz2015connected}. Similar to the design of comprehension test questions in Study 2A, we balanced the difficulty levels of our questions such that 2 were easy, 3 medium, and 3 difficult.
% Except VLAT, we also referenced works of Haroz et al.~\cite{haroz2015connected} that has discussed common misinterpretations of connected scatter plots to design our questions.

The easy questions required participants to retrieve specific values from the connected scatter plot. An example would be ``What was the price of gasoline per gallon in America in 1984?". The medium questions require the participant to find extremes or identify trends. For example, ``From 1970 to 1980, in which year was the average number of miles an American drove per day the highest?" % , and "Between 1985 and 1986, the price of gasoline in America (increased, decreased, not changed) while the average number of miles an American drove per day (increased, decreased, not changed).".
Because viewers tend to have trouble with interpreting backward diagonals in connected scatter plots \cite{haroz2015connected}, we specifically included questions asking our participants to interpret backward trends in our difficult questions, such as ``Name the first pair of consecutive years (e.g., 1970-1971) when the price of gasoline in America increased and the average number of miles an American drove per day decreased." 
We also ensured that the three explanation types would have similar text complexity and length. The specific explanations can be found in the supplementary materials. 

% Referent - In this chart, the line in the middle displays the year information. On the left side, the y-axis indicates the price of gasoline per gallon in America in the year. On the bottom, the x-axis shows the average number of miles an American drove per day in the year. 
% Encoding - 54 In this chart, each dot on the line is associated with data from the labeled year. The vertical position of the dot represents the price of gasoline per gallon in America in the year.  The horizontal position of the dot represents the average number of miles an American drove per day in the year.
% Rule - 57 In this chart, the year increases as you follow the connected dots on the line. A dot further to the top means the price of gasoline per gallon in America was higher during that year.  A dot further to the right means the average number of miles an American drove per day were higher during that year.

\subsection{Results}
We constructed a similar one-way ANOVA comparing participant performance on the comprehension test for the explanation subcategories (reference, encoding, rule). Consistent with the result from Study 2A, we found no significant effects of explanation type on the comprehension test scores ($F = 0.16, p = 0.85 {\eta^2}_{partial} = 0.004$). As shown in \autoref{fig:study2aand3a}, the average comprehension test scores in each explanation type were: referent ($M = 6.43, SD = 1.10$), encoding ($M = 6.21 , SD = 1.47$), and rule ($Mean = 6.30, SD = 1.76$). The referent type yielded the best results, although not significantly. 

We conducted a linear regression analysis predicting performance on the comprehension test with visualization literacy, age, education level, gender as well as the explanation type. Similar to what we observed in Study 2A, visualization literacy is the only predictor significantly influenced participant performance ($coef = 0.066, p = 0.056$), and post-hoc analysis suggest that there is no significant difference in visual literacy levels between the participants who viewed different explanation types ($ F = 0.22, p = 0.80, {\eta^2}_{partial} = 0.005$).
The effects of explanation type, age, gender, and education levels were negligible. Details can be found in the supplementary materials.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Study 3B: Introducing A Connected Scatterplot}
Study 3B follows the same procedure as Study 2B and uses the same comprehension questions as Study 2A. The six introduction types remained the same: explanation only (E), explanation followed by knowledge (EK), explanation interwoven with knowledge (EKEK), indicator followed by explanation (IE), indicator plus explanation followed by knowledge (IEK), and indicator plus explanation interwoven with knowledge (IEKEK). 

In study 2B, we chose the best performing explanation type from Study 2A as the explanation type. To be consistent, we chose the referent type to be the explanation type here in Study 3A, as the referent type encoding led to the highest performance in Study 3A, although not statistically significant. 
For the indicator and knowledge components, we chose \textit{Topic} as the indicator type and selected extreme data values as the knowledge example to stay consistent with Study 2B. The instruction text we generated for Study 3B can be found in the supplementary materials.

We recruited 180 participants (ages ranged between 18 and 70 years old, $\mu = 35.48 , \sigma = 13.42$, $56\%$ females) and collected 169 valid responses after applying the same exclusion criteria as before. % $63\%$ of them never or rarely incorporate data charts/visualizations in their works, $20\%$ sometimes and $17\%$ often or very often. $76\%$ of them rarely or never saw the types of charts in the experiment, $18\%$ sometimes, and $6\%$ often or very often.

\subsection{Results}
We constructed a similar two-way ANOVA as that in Study 2B, comparing the main effects of indicator inclusion (whether an indicator was present or not) and introduction body content (whether knowledge was excluded, included but separated from the explanation, or included and interwoven with the explanation), and the effect of their interaction on participant performance on the comprehension test.

The average comprehension test scores in introduction types are as follows: E (Mean = 6.43, SD = 1.10), IE (Mean =  6.41, SD = 1.34), EK (Mean = 5.93, SD = 1.86), IEK (Mean = 6.16, SD = 1.70), EKEK (Mean = 6.04, SD = 1.76), and IEKEK (Mean = 6.22, SD = 1.55).

Interestingly, we found no main effects of indicator inclusion ($F = 0.27, p = 0.60, {\eta^2}_{partial} = 0.002$) nor introduction body content ($F = 1.01, p = 0.32, {\eta^2}_{partial} = 0.006$).
There was also no significant interaction effect between indicator inclusion and introduction body content ($F = 0.14, p = 0.71, {\eta^2}_{partial} = 0.000$).
This suggests that participants performed similarly regardless of which introduction type they listened to. 

% Although we found participants who listened to introductions that included an indicator (IE, IEK, IEKEK) consistently performing \leni{wrong interpretation} better no matter whether the knowledge component was included or whether the explanation interwoven with knowledge than participants listening to introductions excluding indicator (E, EK, EKEK).

We also conducted a linear regression analysis to examine the effects of visualization literacy, age, education level, gender, indicator inclusion, and introduction body content on the comprehension test scores.
The results show that visualization literacy significantly influenced participant performance ($coef = 0.098, p = 0.000$), such that participants performed better on the comprehension test when they have higher visual literacy levels. 
We also found an effect of age ($coef = -0.019, p = 0.025$) and education level ($coef = 0.255, p = 0.002$). We discuss the implications of these results in comparison with that from Study 2B, in the general discussion section.

% \subsection{Comparing Study2 and Study3} 
% We found the experiment results about connected scatter plot and Mekko chart inconsistent. There is no significant difference between all introductions of connected scatter plot, yet introductions with knowledge component of the Mekko chart significantly improve participant performance than introductions without knowledge component. We suspect that it is because the Mekko chart is more complex than the connected scatter plot for participants. Therefore the participants must rely more on the introductions when understanding the Mekko chart. On the other hand, they could understand most part of the connected scatter plot no matter what the introduction type was based on their prior knowledge. Participants have overall higher performance on the comprehension test for the Mekko chart than for the connected scatter plot, as shown in \leni{figure xxx}. We further discuss it in our Discussion section. \leni{cite the discussion section}
